Causal Modeling with Stationary Diffusions

We develop a novel approach towards causal inference. Rather than structural equations over a causal graph, we learn stochastic differential equations (SDEs) whose stationary densities model a system's behavior under interventions. These stationary diffusion models do not require the formalism of causal graphs, let alone the common assumption of acyclicity. We show that in several cases, they generalize to unseen interventions on their variables, often better than classical approaches. Our inference method is based on a new theoretical result that expresses a stationarity condition on the diffusion's generator in a reproducing kernel Hilbert space. The resulting kernel deviation from stationarity (KDS) is an objective function of independent interest.

==> fig/witness.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{img/witness.pdf}
    \caption{%
    \looseness-1
    Illustration of the KDS and its components for a stationary linear SDE
    and the RKHS of a
    % $\Fcal$ is the unit ball RKHS of the 
    Gaussian kernel $\smash{k_\gamma}$ with $\gamma = 0.5$.
    Expectations over $\mu$ are approximated using $1000$ samples.
    {\em Left:} 
    Probability density functions and parameters of the target ($\mu$, black) and two alternative models (red and blue).
    {\em Center:}
    Witness functions and integrands of the outer KDS integral for the misspecified models. 
    The KDS equals the integral of the shaded areas.
    {\em Right:}
    Partial derivatives of the KDS when varying $a$ and $c$, respectively, fixing the remaining parameters at those of the target model.
    % (see legend).
    True and incorrect parameters of the models are indicated by vertical, dashed lines.
    }
    \label{fig:witness}
\end{figure}

